AGN in overdense environments at high-$z$ with AXIS

Overdense regions at high redshift ($z \gtrsim 2$) are perfect laboratories to study the relations between environment and SMBH growth, and the AGN feedback processes on the surrounding galaxies and diffuse gas. In this white paper, we discuss how AXIS will 1) constrain the AGN incidence in protoclusters, as a function of parameters such as redshift, overdensity, mass of the structure; 2) search for low-luminosity and obscured AGN in the satellite galaxies of luminous QSOs at $z>6$, exploiting the large galaxy density around such biased objects; 3) probe the AGN feedback on the proto-ICM via the measurement of the AGN contribution to the gas ionization and excitation, and the detection of extended X-ray emission from the ionized gas and from radio jets; 4) discover new large-scale structures in the wide and deep AXIS surveys as spikes in the redshift distribution of X-ray sources. These goals can be achieved only with an X-ray mission with the capabilities of AXIS, ensuring a strong synergy with current and future state-of-the-art facilities in other wavelengths. This White Paper is part of a series commissioned for the AXIS Probe Concept Mission; additional AXIS White Papers can be found at http://axis.astro.umd.edu/ with a mission overview at https://arxiv.org/abs/2311.00780.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
